Do LLMs estimate uncertainty well in instruction-following?

Large language models (LLMs) could be valuable personal AI agents across various domains, provided they can precisely follow user instructions. However, recent studies have shown significant limitations in LLMs' instruction-following capabilities, raising concerns about their reliability in high-stakes applications. Accurately estimating LLMs' uncertainty in adhering to instructions is critical to mitigating deployment risks. We present, to our knowledge, the first systematic evaluation of the uncertainty estimation abilities of LLMs in the context of instruction-following. Our study identifies key challenges with existing instruction-following benchmarks, where multiple factors are entangled with uncertainty stems from instruction-following, complicating the isolation and comparison across methods and models. To address these issues, we introduce a controlled evaluation setup with two benchmark versions of data, enabling a comprehensive comparison of uncertainty estimation methods under various conditions. Our findings show that existing uncertainty methods struggle, particularly when models make subtle errors in instruction following. While internal model states provide some improvement, they remain inadequate in more complex scenarios. The insights from our controlled evaluation setups provide a crucial understanding of LLMs' limitations and potential for uncertainty estimation in instruction-following tasks, paving the way for more trustworthy AI agents.

==> contents/FT.tex <==
\section{Fine-Tuning}
\textbf{Setups}
Epoch, data, model. We set ground-truth label as 0, 4.5, 9.

Result: Better than before (verbal score). Plot PCA if available. 


==> contents/RwE.tex <==
\section{Do internal states of LLMs know more about their uncertainty?}\label{sec:RwE}
In the previous section, we demonstrated that both self-evaluation and logit-based methods performed poorly in the Controlled-Hard setting, where instruction-following mistakes were subtle. AUROC for uncertainty estimation was often below 0.6. Drawing inspiration from \cite{liu2024uncertainty}, which suggests that model representations contain valuable information for uncertainty estimation in tasks like question and answering, we investigated whether this internal knowledge could similarly improve uncertainty estimation in instruction-following tasks.
We trained a linear model as an uncertainty estimation function that maps the internal representations of LLMs to instruction-following success labels, where the probability predicted by the linear model used as uncertainty scores. 
% reflecting the model's confidence in its responses within the context of instruction-following. 
% The probability predicted by the linear model was used as the uncertainty score. 
The ground truth for success or failure is determined by a deterministic program that verifies instruction adherence using the IFEval dataset. We refer to this as \textbf{Probe}. 
% (described in Section 2.1). 



% We train a linear model as an uncertainty estimation function that maps the internal representations of LLMs to an uncertainty score that captures LLMs confidence about its response in context of instruction-following. 
% In supervised way, we train a linear model on the internal representations of LLMs and instruction-following success labels, which are determined by a deterministic program that verifies instruction adherence using the IFEval dataset (described in Section 2.1).
% % The ground truth for success or failure is determined by a deterministic program that verifies instruction adherence using the IFEval dataset (described in Section 2.1). 
% We refer to this as \textbf{Probe}.
% to classify instruction-following success or failure. 
% The ground truth for success or failure is determined by a deterministic program that verifies instruction adherence using the IFEval dataset (described in Section 2.1). 


\subsection{Settings}
\textbf{Representations}
We analyzed four language models: LLaMA-2-7B-chat, LLaMA-2-13B-chat, Mistral-7B-Instruct-v0.3, and Phi-3-mini-128k-instruct. For each model, we collected representations across three different layers: early, middle, and the final layer. Specifically, we use layers 16, 32, and 40 and for LLaMA-2-13B-chat and 14, 26, and 32 for other three models. 

\textbf{Linear Model and metric}
We train a linear model on representations on instruction-following success labels, optimized with AdamW, a 0.001 learning rate, 0.1 weight decay. The model is trained for 1000 epochs on 70\% training set and is evaluated on 30\% test set. We use AUROC as metric.
% to assess the performance of binary prediction.




\subsection{Results}
\textbf{Probe generally outperformed baseline methods in both Controlled-Easy and Realistic version}, as shown in Table \ref{tab:benchmark_simple_ver}. 
Probe consistently outperformed even self-evaluation methods such as berbalized confidence and normalized-p(true).
This gap between what the internal states of the model ``know'' and what they are able to express suggests that their internal layers hold richer, more reliable indicators of uncertainty, which are not fully captured in the model's explicit responses.
This points to promising directions for future work, specifically in improving self-evaluation methods by leveraging the rich information within a model’s internal representations. 

\textbf{Middle layers consistently offer the most informative representations for uncertainty estimation}, particularly in simpler tasks (Controlled-Easy). Appendix Table \ref{tab:probe_split} shows how Probe performance varies across instruction types and layers within the LLMs. The middle layers consistently provide the best signals for uncertainty, indicating that future work could focus on extracting more refined signals from these middle layers to enhance uncertainty estimation methods. 

\textbf{Probe still struggles with uncertainty estimation in more challenging scenarios.} In Controlled-Hard, Probe AUROC scores drop below 0.60 across all models, revealing that even the internal representations struggle to estimate uncertainty accurately when the task complexity increases. 
This suggests a limitation in LLMs’ ability to handle nuanced or complex uncertainty, highlighting the need for further model fine-tuning or the development of more sophisticated uncertainty estimation methods to improve uncertainty estimation in these difficult tasks.






==> contents/discussion.tex <==
\section{Discussion}

==> contents/milestones.tex <==
\section*{Milestones}
\subsection{Write skeleton: one for a day}
\begin{itemize}
    \item \sout{2,3: Generate experiment tables}
    \item \sout{Tue: Write introduction skeleton + contributions (sec 1)}
    \item \sout{4: Write ifeval skeleton (sec 2)}
    \item \sout{5: Write Benchmark skeleton (sec 3)}
    \item \sout{7: Write RwE skeleton (sec 4) + Write FT skeleton (sec 5) + Write Related work skeleton (sec 6)}
    \item \sout{8: Write Discussion \& Conclusion skeleton (sec 7, 8)}
\end{itemize}

\subsection{Write draft: one for a day}
\begin{itemize}
    \item 11: Write introduction draft + contributions (sec 1)
    \item 12: Draw Figure 1 + Write ifeval draft (sec 2) + Write Benchmark draft (sec 3)
    \item 13: Write RwE draft (sec 4)
    \item 14: Write FT draft (sec 5)
    \item 15: Write Related work draft (sec 6)
    \item 16: Write Discussion \& Conclusion draft (sec 7, 8) + polish figures
\end{itemize}

\subsection{Share: Jaya, Chritina, Shierly}

\subsection{Polishing draft: one for a day}
\begin{itemize}
    \item 17: Write ifeval polish (sec 2) + Write Benchmark polish (sec 3)
    \item \sout{18: sec 2}
    \item \sout{19: sec 4}
    \item \sout{20: sec 5}
    \item 21: sec 3
    \item 22: sec 6: related work
\end{itemize}

\subsection{Share: Jaya, Chritina, Shierly and others}

\subsection{Refinement: one for a day}
\begin{itemize}
    \item 22: Write ifeval Refinement (sec 2) + Write Benchmark Refinement (sec 3)
    \item 23: Write RwE Refinement (sec 4) + Write FT Refinement (sec 5)
    \item 24: Write FT Refinement (sec 5) + Write Related work Refinement (sec 6)
    \item 25: Write Discussion \& Conclusion Refinement (sec 7, 8) +  Write introduction Refinement + contributions (sec 1)
    \item 26: Refine Appendix
\end{itemize}


\subsection{Submit Apple internal}

==> contents/table/RwE_versionB.tex <==

% \begin{table}[H]
% \centering
% \resizebox{0.6\textwidth}{!}{%
% \begin{tabular}{@{}l|l|ccc|ccc@{}}
% \toprule
% \textbf{Model} & \textbf{Instructions} & \multicolumn{3}{c|}{\textbf{Linear, 60-40 split}} & \multicolumn{3}{c}{\textbf{Projection 1dim, training set}} \\ \midrule
% & & \multicolumn{6}{c}{\textbf{Realistic}}\\ \midrule
%  &  & \textbf{Early} & \textbf{Middle} & \textbf{Last} & \textbf{Early} & \textbf{Middle} & \textbf{Last} \\ \midrule
% \multirow{9}{*}{7B model} 
%  & startend & 0.84 & 0.85 & 0.70 & 0.79 & 0.75 & 0.74 \\
%  & detectable\_content & 0.93 & 0.73 & 0.44 & 0.44 & 0.51 & 0.51 \\
%  & detectable\_format & 0.57 & 0.58 & 0.59 & 0.60 & 0.61 & 0.61 \\
%  & language & 0.33 & 0.67 & 0.50 & 0.67 & 0.67 & 0.67 \\
%  & change\_case & 0.60 & 0.60 & 0.58 & 0.49 & 0.55 & 0.57 \\
%  & keywords & 0.56 & 0.61 & 0.46 & 0.58 & 0.59 & 0.60 \\
%  & length\_constraints & 0.53 & 0.42 & 0.51 & 0.56 & 0.57 & 0.57 \\
%  & punctuation & 0.44 & 0.44 & 1.00 & 0.84 & 0.86 & 0.86 \\
%  & \textbf{Average} & 0.60 & 0.61 & 0.60 & 0.62 & 0.64 & 0.64 \\ \midrule

% \multirow{9}{*}{13B model} 
%  & startend & 0.74 & 0.83 & 0.80 & 0.81 & 0.82 & 0.84 \\
%  & detectable\_content & 0.63 & 0.44 & 0.56 & 0.55 & 0.57 & 0.53 \\
%  & detectable\_format & 0.54 & 0.58 & 0.51 & 0.62 & 0.61 & 0.61 \\
%  & language & 1.00 & 1.00 & 0.50 & 0.78 & 0.83 & 0.83 \\
%  & change\_case & 0.55 & 0.39 & 0.51 & 0.52 & 0.54 & 0.55 \\
%  & keywords & 0.54 & 0.55 & 0.46 & 0.57 & 0.58 & 0.59 \\
%  & length\_constraints & 0.63 & 0.59 & 0.56 & 0.59 & 0.62 & 0.63 \\
%  & punctuation & 0.78 & 0.75 & 1.00 & 0.84 & 0.80 & 0.82 \\
%  & \textbf{Average} & 0.68 & 0.64 & 0.61 & 0.66 & 0.67 & 0.67 \\ \midrule

% \multirow{9}{*}{\shortstack{Mistral-7B-\\Instruct-v0.3}} 
%  & startend & 0.54 & 0.53 & 0.76 & 0.79 & 0.78 & 0.65 \\
%  & detectable\_content & 0.81 & 0.63 & 0.60 & 0.43 & 0.47 & 0.44 \\
%  & detectable\_format & 0.52 & 0.59 & 0.59 & 0.61 & 0.60 & 0.57 \\
%  & language & 1.00 & 1.00 & 0.59 & 0.72 & 0.67 & 0.61 \\
%  & change\_case & 0.44 & 0.48 & 0.43 & 0.48 & 0.46 & 0.46 \\
%  & keywords & 0.59 & 0.66 & 0.58 & 0.62 & 0.66 & 0.64 \\
%  & length\_constraints & 0.49 & 0.60 & 0.53 & 0.59 & 0.60 & 0.59 \\
%  & punctuation & 0.78 & 0.78 & 0.88 & 0.78 & 0.88 & 0.76 \\
%  & \textbf{Average} & 0.65 & 0.66 & 0.62 & 0.63 & 0.64 & 0.59 \\ \midrule

% \multirow{9}{*}{\shortstack{Phi-3-mini-\\128k-instruct}}
%  & startend & 0.80 & 0.89 & 0.93 & 0.80 & 0.76 & 0.69 \\
%  & detectable\_content & 0.93 & 0.81 & 0.92 & 0.59 & 0.62 & 0.53 \\
%  & detectable\_format & 0.50 & 0.52 & 0.49 & 0.61 & 0.66 & 0.65 \\
%  & language & 1.00 & 1.00 & 0.67 & 0.78 & 0.89 & 0.72 \\
%  & change\_case & 0.46 & 0.51 & 0.46 & 0.49 & 0.51 & 0.49 \\
%  & keywords & 0.72 & 0.49 & 0.43 & 0.54 & 0.60 & 0.61 \\
%  & length\_constraints & 0.60 & 0.62 & 0.73 & 0.60 & 0.62 & 0.61 \\
%  & punctuation & 0.44 & 0.89 & 0.67 & 0.73 & 0.78 & 0.69 \\
%  & \textbf{Average} & 0.68 & 0.72 & 0.66 & 0.64 & 0.68 & 0.62 \\ \bottomrule
% \end{tabular}
% }
% \caption{RwE metrics for different models and instructions, showing early, middle, and late layer performance in both linear and projection methods.}
% \label{table:combined}
% \end{table}

\begin{table}[H]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}l|l|ccc|ccc|ccc@{}}
\toprule
& & \multicolumn{3}{c|}{\textbf{Controlled-Easy}} & \multicolumn{3}{c|}{\textbf{Controlled-Hard}}& \multicolumn{3}{c}{\textbf{Realistic}} \\\midrule
 \textbf{Model} & \textbf{Instructions} & \textbf{Early} & \textbf{Middle} & \textbf{Last} & \textbf{Early} & \textbf{Middle} & \textbf{Last} & \textbf{Early} & \textbf{Middle} & \textbf{Last} \\ \hline
\multirow{9}{*}{LLaMA-2-chat-7B} 
 & startend & 0.58 & 0.64 & 0.63 & 0.60 & 0.61 & 0.60 & 0.79 & 0.75 & 0.74 \\
 & detectable\_content & 0.65 & 0.69 & 0.67 & 0.58 & 0.57 & 0.57 & 0.44 & 0.51 & 0.51 \\
 & detectable\_format & 0.63 & 0.62 & 0.62 & 0.61 & 0.60 & 0.58 & 0.60 & 0.61 & 0.61 \\
 & language & 0.80 & 0.77 & 0.74 & 0.80 & 0.65 & 0.62 & 0.67 & 0.67 & 0.67 \\
 & change\_case & 0.55 & 0.59 & 0.60 & 0.59 & 0.59 & 0.57 & 0.49 & 0.55 & 0.57 \\
 & keywords & 0.54 & 0.66 & 0.69 & 0.54 & 0.60 & 0.63 & 0.58 & 0.59 & 0.60 \\
 & length\_constraints & 0.58 & 0.68 & 0.70 & 0.64 & 0.63 & 0.63 & 0.56 & 0.57 & 0.57 \\
 & punctuation & 0.45 & 0.51 & 0.52 & 0.53 & 0.50 & 0.50 & 0.84 & 0.86 & 0.86 \\\cline{2-11} 
 & \textbf{Average} & 0.60 & 0.65 & 0.64 & 0.61 & 0.59 & 0.59 & 0.62 & 0.64 & 0.64 \\ \midrule

\multirow{9}{*}{LLaMA-2-chat-13B} 
 & startend & 0.67 & 0.68 & 0.68 & 0.59 & 0.57 & 0.58 & 0.81 & 0.82 & 0.84 \\
 & detectable\_content & 0.73 & 0.74 & 0.74 & 0.63 & 0.52 & 0.53 & 0.55 & 0.57 & 0.53 \\
 & detectable\_format & 0.70 & 0.70 & 0.70 & 0.61 & 0.63 & 0.62 & 0.62 & 0.61 & 0.61 \\
 & language & 0.80 & 0.78 & 0.77 & 0.94 & 0.84 & 0.82 & 0.78 & 0.83 & 0.83 \\
 & change\_case & 0.60 & 0.63 & 0.63 & 0.60 & 0.55 & 0.55 & 0.52 & 0.54 & 0.55 \\
 & keywords & 0.66 & 0.79 & 0.80 & 0.62 & 0.68 & 0.68 & 0.57 & 0.58 & 0.59 \\
 & length\_constraints & 0.69 & 0.74 & 0.74 & 0.71 & 0.66 & 0.67 & 0.59 & 0.62 & 0.63 \\
 & punctuation & 0.57 & 0.59 & 0.60 & 0.45 & 0.54 & 0.56 & 0.84 & 0.80 & 0.82 \\\cline{2-11} 
 & \textbf{Average} & 0.68 & 0.71 & 0.71 & 0.64 & 0.62 & 0.62 & 0.66 & 0.67 & 0.67 \\ \midrule

\multirow{9}{*}{Mistral-7B-Instruct-v0.3}
 & startend & 0.71 & 0.72 & 0.71 & 0.62 & 0.59 & 0.55 & 0.79 & 0.78 & 0.65 \\
 & detectable\_content & 0.71 & 0.72 & 0.71 & 0.56 & 0.52 & 0.52 & 0.43 & 0.47 & 0.44 \\
 & detectable\_format & 0.73 & 0.76 & 0.77 & 0.64 & 0.65 & 0.62 & 0.61 & 0.60 & 0.57 \\
 & language & 0.84 & 0.65 & 0.67 & 0.86 & 0.76 & 0.69 & 0.72 & 0.67 & 0.61 \\
 & change\_case & 0.62 & 0.71 & 0.70 & 0.67 & 0.53 & 0.50 & 0.48 & 0.46 & 0.46 \\
 & keywords & 0.67 & 0.89 & 0.89 & 0.60 & 0.73 & 0.73 & 0.62 & 0.66 & 0.64 \\
 & length\_constraints & 0.82 & 0.86 & 0.84 & 0.61 & 0.53 & 0.56 & 0.59 & 0.60 & 0.59 \\
 & punctuation & 0.66 & 0.68 & 0.65 & 0.60 & 0.57 & 0.53 & 0.78 & 0.88 & 0.76 \\\cline{2-11} 
 & \textbf{Average} & 0.72 & 0.75 & 0.74 & 0.65 & 0.61 & 0.59 & 0.63 & 0.64 & 0.59 \\ \midrule

\multirow{9}{*}{Phi-3-mini-128k-instruct}
 & startend & 0.71 & 0.75 & 0.75 & 0.62 & 0.66 & 0.63 & 0.80 & 0.76 & 0.69 \\
 & detectable\_content & 0.71 & 0.76 & 0.76 & 0.53 & 0.53 & 0.55 & 0.59 & 0.62 & 0.53 \\
 & detectable\_format & 0.75 & 0.75 & 0.74 & 0.61 & 0.66 & 0.65 & 0.61 & 0.66 & 0.65 \\
 & language & 0.86 & 0.62 & 0.63 & 0.81 & 0.71 & 0.61 & 0.78 & 0.89 & 0.72 \\
 & change\_case & 0.55 & 0.63 & 0.61 & 0.64 & 0.56 & 0.54 & 0.49 & 0.51 & 0.49 \\
 & keywords & 0.74 & 0.82 & 0.82 & 0.60 & 0.62 & 0.61 & 0.54 & 0.60 & 0.61 \\
 & length\_constraints & 0.74 & 0.82 & 0.82 & 0.64 & 0.74 & 0.74 & 0.60 & 0.62 & 0.61 \\
 & punctuation & 0.59 & 0.67 & 0.67 & 0.60 & 0.60 & 0.59 & 0.73 & 0.78 & 0.69 \\\cline{2-11} 
 & \textbf{Average} & 0.70 & 0.73 & 0.73 & 0.64 & 0.64 & 0.63 & 0.64 & 0.68 & 0.62 \\ \bottomrule
\end{tabular}%
}
\caption{RwE metrics for different models and instructions, showing early, middle, and late layer performance in the "Projection 1dim, training set".}
\label{tab:projection_1dim_training_set}
\end{table}







==> contents/table/length_bias.tex <==


%%%%%%%%%%
% \begin{table}[H]
% \centering
% \resizebox{0.6\columnwidth}{!}{%
% \begin{tabular}{l|ll}
% \toprule
% \textbf{Length of responses (token)} & \textbf{correct} & \textbf{wrong} \\\midrule
% 7b & $241.34 \pm 181.00$ & $298.47 \pm 177.91$ \\
% 13b & $275.22 \pm 190.57$ & $287.36 \pm 177.74$ \\
% 70b & $224.98 \pm 180.01$ & $268.99 \pm 181.24$ \\
% mistral & $250.58 \pm 189.78$ & $257.59 \pm 178.88$ \\
% phi3 & $566.59 \pm 240.22$ & $613.86 \pm 223.58$ \\\midrule
% Our benchmark A (GPT4) & $232.10 \pm 171.29$ & $232.47 \pm 277.80$ \\
% Our benchmark B (all models) & $276.34 \pm 208.70$ & $327.30 \pm 216.19$ \\\bottomrule
% \end{tabular}
% }
% \caption{Length of responses of different models. Correct responses are longer than wrong responses. In TrustfulQA test, correct responses are shorter than wrong ones. In this paper, hallucination responses are longer than correct ones. Here, we don’t have a correctness (task is writing a story). Question: Should we utilize those length biases or remove them in our benchmark? Some papers suggest collecting false/correct cases from real answers from multiple models to keep useful bias. Sub-benchmark Version A) GPT4 correct, wrong, confusing Version B) 7b, 13b, 70b model’s real correct and false responses (+GPT4 filter as well).}
% \label{tab:length_bias}
% \end{table}

%%%%%%%%%%

%%%%%%%%%%
\begin{table}[h]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{lccccccc}
\toprule
\textbf{Data} & \textbf{7b} & \textbf{13b} & \textbf{70b} & \textbf{Mistral} & \textbf{Phi3} & \textbf{Benchmark A (GPT4)} & \textbf{Benchmark B (all models)} \\
\midrule
\textbf{Correct (tokens)} & $241.34 \pm 181.00$ & $275.22 \pm 190.57$ & $224.98 \pm 180.01$ & $250.58 \pm 189.78$ & $566.59 \pm 240.22$ & $232.10 \pm 171.29$ & $276.34 \pm 208.70$ \\
\textbf{Wrong (tokens)} & $298.47 \pm 177.91$ & $287.36 \pm 177.74$ & $268.99 \pm 181.24$ & $257.59 \pm 178.88$ & $613.86 \pm 223.58$ & $232.47 \pm 277.80$ & $327.30 \pm 216.19$ \\
\bottomrule
\end{tabular}
}
\caption{Length(number of tokens) of responses of different models and our two versions of benchmark data}
\label{tab:length_bias}
\end{table}







% \begin{table}[]
% \resizebox{0.8\columnwidth}{!}{%
% \begin{tabular}{l|lll}
% \toprule
% Length of responses(token)  & correct                                 & wrong                                  & confusing \\\midrule
% 7b                 &  299.42 $\pm$ 177.89 &  240.60 $\pm$ 180.68 &               - \\
% 13b                &  287.36 $\pm$ 177.74 &  275.22 $\pm$ 190.57 &               - \\
% 70b                &  268.99 $\pm$ 181.24 &  224.98 $\pm$ 180.01 &               - \\
% mistral            &  397.35 $\pm$ 1045.91 &  250.58 $\pm$ 189.78 &               - \\
% phi3               &  613.86 $\pm$ 223.58 &  602.31 $\pm$ 564.73 &               - \\\midrule
% Our benchmark-A  &  232.10 $\pm$ 171.29 &  232.47 $\pm$ 277.80 &  236.87 $\pm$ 176.30 \\
% Our benchmark-B  &  327.30 $\pm$ 216.19 &  276.34 $\pm$ 208.70 &                                     \\ \bottomrule
% \end{tabular}
% }
% \caption{Length of responses of different models
% Interesting. Correct responses are longer than wrong responses. In TrustfulQA test, correct responses are shorter than wrong one. In this paper, hallucination responses are longer than correct one. Here, we don’t have a correctness (task is writing a story).  
% Question; Should we utilize those length bias? or removing it in our benchmark? — some papers 
% Try: Collecting false/correct cases from real answers from multiple models - to keep useful bias? //
% Sub-benchmark Version A) GPT4 correct, wrong, confusing Version B) 7b, 13, 70b model’s real correct and false responses(+gpt4 filter as well)
% }
% \label{tab:length_bias}
% \end{table}

% \begin{table}[]
% \resizebox{0.6\columnwidth}{!}{%
% \begin{tabular}{l|ll}
% \toprule
% Length of responses(token)  & correct                                 & wrong                               \\\midrule
% 7b                 &  299.42 $\pm$ 177.89 &  240.60 $\pm$ 180.68                 \\
% 13b                &  287.36 $\pm$ 177.74 &  275.22 $\pm$ 190.57                 \\
% 70b                &  268.99 $\pm$ 181.24 &  224.98 $\pm$ 180.01                \\
% mistral            &  397.35 $\pm$ 1045.91 &  250.58 $\pm$ 189.78                 \\
% phi3               &  613.86 $\pm$ 223.58 &  602.31 $\pm$ 564.73                 \\\midrule
% Our benchmark-A  &  232.10 $\pm$ 171.29 &  232.47 $\pm$ 277.80    \\
% Our benchmark-B  &  327.30 $\pm$ 216.19 &  276.34 $\pm$ 208.70                                      \\ \bottomrule
% \end{tabular}
% }
% \caption{Length of responses of different models
% Interesting. Correct responses are longer than wrong responses. In TrustfulQA test, correct responses are shorter than wrong one. In this paper, hallucination responses are longer than correct one. Here, we don’t have a correctness (task is writing a story).  
% Question; Should we utilize those length bias? or removing it in our benchmark? — some papers 
% Try: Collecting false/correct cases from real answers from multiple models - to keep useful bias? //
% Sub-benchmark Version A) GPT4 correct, wrong, confusing Version B) 7b, 13, 70b model’s real correct and false responses(+gpt4 filter as well)
% }
% \label{tab:length_bias}
% \end{table}

==> contents/table/stats_versionB_models.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[]
\begin{tabular}{@{}l|ll@{}}
\toprule
        & \multicolumn{2}{l}{Version B} \\
        & wrong        & correct        \\ \midrule
7b      & 68           & 69             \\
13b     & 72           & 74             \\
70b     & 65           & 98             \\
mistral & 78           & 87             \\
phi     & 62           & 41             \\ \midrule
Total   & 345          & 369        \\ \bottomrule   
\end{tabular}
\end{table}

==> contents/table/summary_dataset_comparison.tex <==
% \begin{table}[h!]
% \centering
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{lccc}
% \toprule
% \textbf{Criteria} & \textbf{Own Responses} & \textbf{Version A} & \textbf{Version B} \\
% \midrule
% Length Bias-Free & ✗ & ✓ & ✗ \\
% Disentanglement from Task Quality & ✗ & ✓ & ✓ \\
% Controlled Difficulty in Distinguishing Correct and Incorrect Responses & ✗ & ✓ & ✓ \\
% Balanced Correct and Incorrect Responses Across Instructions & ✗ & ✓ & ✓ \\
% \bottomrule
% \end{tabular}
% }
% \caption{Comparison of Criteria Across Different Response Versions}
% \label{tab:summary_data_comparison}
% \end{table}


\begin{table}%[h!]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{lccc}
\toprule
\textbf{Criteria} & \textbf{Own Responses} & \textbf{Version A} & \textbf{Version B} \\
\midrule
Length Bias-Free & \ding{55} & \ding{51} & \ding{55} \\
Disentanglement from Task Quality & \ding{55} & \ding{51} & \ding{51} \\
Controlled Difficulty in Distinguishing Correct and Incorrect Responses & \ding{55} & \ding{51} & \ding{51} \\
Balanced Correct and Incorrect Responses Across Instructions & \ding{55} & \ding{51} & \ding{51} \\
\bottomrule
\end{tabular}
}
\caption{Comparison of Criteria Across Different Response Versions}
\label{tab:summary_data_comparison}
\end{table}



==> contents/table/versionA_uncertainty.tex <==

\begin{table}%[h!]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}l|l|cccccc|cccccc@{}}
\toprule
\textbf{Metric: AUROC} & \textbf{Model} & \multicolumn{6}{c|}{\textbf{Version A-Easy}} & \multicolumn{6}{c}{\textbf{Version A-Hard}} \\ \midrule
 & \textbf{Instructions} & \textbf{Verbal} & \textbf{Perplexity} & \textbf{Max-seq} & \textbf{Nor-p(true)} & \textbf{p(true)} & \textbf{Entropy} & \textbf{Verbal} & \textbf{Perplexity} & \textbf{Max-seq} & \textbf{Nor-p(true)} & \textbf{p(true)} & \textbf{Entropy} \\ \midrule
\multirow{9}{*}{\textbf{7B model}} & startend & 0.64 & 0.59 & 0.50 & 0.55 & 0.43 & 0.55 & 0.52 & 0.57 & 0.54 & 0.49 & 0.43 & 0.56 \\
 & detectable\_content & 0.65 & 0.63 & 0.49 & 0.53 & 0.41 & 0.56 & 0.52 & 0.58 & 0.52 & 0.49 & 0.43 & 0.55 \\
 & detectable\_format & 0.61 & 0.62 & 0.48 & 0.53 & 0.44 & 0.57 & 0.51 & 0.58 & 0.52 & 0.51 & 0.45 & 0.54 \\
 & language & 0.63 & 0.62 & 0.46 & 0.52 & 0.43 & 0.54 & 0.51 & 0.59 & 0.51 & 0.50 & 0.45 & 0.52 \\
 & change\_case & 0.63 & 0.60 & 0.47 & 0.54 & 0.46 & 0.52 & 0.52 & 0.57 & 0.50 & 0.51 & 0.45 & 0.53 \\
 & keywords & 0.65 & 0.61 & 0.49 & 0.55 & 0.48 & 0.52 & 0.54 & 0.57 & 0.51 & 0.52 & 0.47 & 0.52 \\
 & length\_constraints & 0.66 & 0.60 & 0.49 & 0.56 & 0.48 & 0.51 & 0.55 & 0.57 & 0.51 & 0.52 & 0.47 & 0.53 \\
 & punctuation & 0.65 & 0.60 & 0.50 & 0.56 & 0.49 & 0.52 & 0.55 & 0.57 & 0.51 & 0.51 & 0.47 & 0.53 \\\cline{2-14} 
 & \textbf{Average} & 0.64 & 0.61 & 0.48 & 0.54 & 0.45 & 0.54 & 0.53 & 0.57 & 0.51 & 0.51 & 0.45 & 0.53 \\ \midrule
\multirow{9}{*}{\textbf{13B model}} & startend & 0.65 & 0.58 & 0.50 & 0.67 & 0.44 & 0.58 & 0.52 & 0.58 & 0.54 & 0.56 & 0.43 & 0.59 \\
 & detectable\_content & 0.67 & 0.63 & 0.49 & 0.64 & 0.48 & 0.59 & 0.50 & 0.59 & 0.51 & 0.54 & 0.44 & 0.56 \\
 & detectable\_format & 0.66 & 0.62 & 0.48 & 0.59 & 0.45 & 0.59 & 0.51 & 0.61 & 0.52 & 0.53 & 0.43 & 0.58 \\
 & language & 0.67 & 0.64 & 0.46 & 0.59 & 0.44 & 0.60 & 0.53 & 0.62 & 0.51 & 0.53 & 0.42 & 0.57 \\
 & change\_case & 0.66 & 0.62 & 0.47 & 0.59 & 0.46 & 0.56 & 0.51 & 0.60 & 0.50 & 0.51 & 0.43 & 0.57 \\
 & keywords & 0.68 & 0.62 & 0.49 & 0.61 & 0.46 & 0.56 & 0.53 & 0.60 & 0.51 & 0.53 & 0.45 & 0.56 \\
 & length\_constraints & 0.68 & 0.61 & 0.50 & 0.62 & 0.46 & 0.55 & 0.55 & 0.59 & 0.52 & 0.55 & 0.45 & 0.56 \\
 & punctuation & 0.68 & 0.61 & 0.50 & 0.61 & 0.46 & 0.56 & 0.54 & 0.59 & 0.52 & 0.54 & 0.45 & 0.56 \\\cline{2-14} 
 & \textbf{Average} & 0.67 & 0.62 & 0.48 & 0.61 & 0.46 & 0.57 & 0.52 & 0.60 & 0.52 & 0.54 & 0.44 & 0.57 \\ \midrule
\multirow{9}{*}{\shortstack{Mistral-7B-\\Instruct-v0.3}}  & startend & 0.69 & 0.59 & 0.46 & 0.64 & 0.46 & 0.47 & 0.54 & 0.54 & 0.51 & 0.56 & 0.43 & 0.46 \\
 & detectable\_content & 0.70 & 0.60 & 0.43 & 0.65 & 0.46 & 0.46 & 0.53 & 0.56 & 0.49 & 0.54 & 0.45 & 0.48 \\
 & detectable\_format & 0.71 & 0.63 & 0.44 & 0.66 & 0.48 & 0.45 & 0.56 & 0.57 & 0.49 & 0.57 & 0.48 & 0.48 \\
 & language & 0.71 & 0.61 & 0.41 & 0.67 & 0.49 & 0.41 & 0.56 & 0.55 & 0.48 & 0.56 & 0.49 & 0.44 \\
 & change\_case & 0.70 & 0.57 & 0.43 & 0.65 & 0.49 & 0.42 & 0.56 & 0.54 & 0.48 & 0.54 & 0.50 & 0.45 \\
 & keywords & 0.72 & 0.58 & 0.45 & 0.66 & 0.49 & 0.40 & 0.58 & 0.54 & 0.49 & 0.55 & 0.50 & 0.45 \\
 & length\_constraints & 0.73 & 0.58 & 0.45 & 0.68 & 0.48 & 0.41 & 0.59 & 0.55 & 0.49 & 0.57 & 0.50 & 0.45 \\
 & punctuation & 0.73 & 0.58 & 0.46 & 0.67 & 0.49 & 0.41 & 0.58 & 0.55 & 0.49 & 0.57 & 0.49 & 0.45 \\\cline{2-14} 
 & \textbf{Average} & 0.71 & 0.59 & 0.44 & 0.66 & 0.48 & 0.43 & 0.56 & 0.55 & 0.49 & 0.56 & 0.48 & 0.46 \\ \midrule
\multirow{9}{*}{\shortstack{Phi-3-mini-\\128k-instruct}}   & startend & 0.62 & 0.59 & 0.47 & 0.74 & 0.53 & 0.56 & 0.56 & 0.55 & 0.46 & 0.64 & 0.40 & 0.50 \\
 & detectable\_content & 0.66 & 0.64 & 0.40 & 0.71 & 0.55 & 0.58 & 0.53 & 0.55 & 0.44 & 0.59 & 0.43 & 0.49 \\
 & detectable\_format & 0.64 & 0.57 & 0.41 & 0.73 & 0.53 & 0.57 & 0.55 & 0.52 & 0.48 & 0.62 & 0.47 & 0.53 \\
 & language & 0.63 & 0.58 & 0.41 & 0.72 & 0.55 & 0.57 & 0.55 & 0.52 & 0.47 & 0.61 & 0.49 & 0.52 \\
 & change\_case & 0.62 & 0.56 & 0.41 & 0.70 & 0.57 & 0.55 & 0.55 & 0.50 & 0.47 & 0.59 & 0.51 & 0.53 \\
 & keywords & 0.65 & 0.59 & 0.39 & 0.72 & 0.59 & 0.54 & 0.56 & 0.52 & 0.48 & 0.61 & 0.52 & 0.52 \\
 & length\_constraints & 0.65 & 0.58 & 0.41 & 0.73 & 0.58 & 0.53 & 0.57 & 0.53 & 0.48 & 0.61 & 0.52 & 0.00 \\
 & punctuation & 0.65 & 0.57 & 0.43 & 0.73 & 0.58 & 0.54 & 0.57 & 0.53 & 0.48 & 0.63 & 0.52 & 0.52 \\\cline{2-14} 
 & \textbf{Average} & 0.64 & 0.58 & 0.42 & 0.72 & 0.56 & 0.55 & 0.55 & 0.53 & 0.47 & 0.62 & 0.48 & 0.52 \\ \bottomrule
\end{tabular}
}
\caption{AUROC metrics for different models, instructions, and uncertainty methods, showing both easy and confusing cases.}
\label{tab:versionA}
\end{table}

==> contents/table/versionB_uncertainty.tex <==

\begin{table}[h!]
\centering
\resizebox{0.8\textwidth}{!}{%
\begin{tabular}{@{}l|l|cccccc@{}}
\toprule
\textbf{Metric: AUROC} & \textbf{Model} & \multicolumn{6}{c|}{\textbf{Version B}} \\ \midrule
\textbf{Model} & \textbf{Instructions} & \textbf{Verbal} & \textbf{Perplexity} & \textbf{Max-seq} & \textbf{Nor-p(true)} & \textbf{p(true)} & \textbf{Entropy} \\ \midrule
\multirow{9}{*}{7B model} 
 & startend & 0.41 & 0.52 & 0.74 & 0.54 & 0.44 & 0.46 \\
 & detectable\_content & 0.43 & 0.55 & 0.72 & 0.52 & 0.42 & 0.50 \\
 & detectable\_format & 0.50 & 0.50 & 0.60 & 0.54 & 0.48 & 0.51 \\
 & language & 0.49 & 0.50 & 0.61 & 0.53 & 0.48 & 0.50 \\
 & change\_case & 0.50 & 0.49 & 0.57 & 0.53 & 0.48 & 0.50 \\
 & keywords & 0.51 & 0.50 & 0.57 & 0.53 & 0.49 & 0.50 \\
 & length\_constraints & 0.51 & 0.50 & 0.56 & 0.51 & 0.48 & 0.50 \\
 & punctuation & 0.51 & 0.50 & 0.57 & 0.51 & 0.48 & 0.51 \\\cline{2-8}
 & \textbf{Average} & 0.48 & 0.51 & 0.62 & 0.53 & 0.47 & 0.50 \\ \midrule

\multirow{9}{*}{13B model} 
 & startend & 0.52 & 0.49 & 0.67 & 0.53 & 0.54 & 0.40 \\
 & detectable\_content & 0.52 & 0.53 & 0.67 & 0.54 & 0.52 & 0.44 \\
 & detectable\_format & 0.51 & 0.53 & 0.62 & 0.54 & 0.46 & 0.48 \\
 & language & 0.50 & 0.52 & 0.62 & 0.53 & 0.46 & 0.47 \\
 & change\_case & 0.51 & 0.51 & 0.58 & 0.51 & 0.46 & 0.47 \\
 & keywords & 0.52 & 0.51 & 0.57 & 0.51 & 0.47 & 0.48 \\
 & length\_constraints & 0.51 & 0.51 & 0.57 & 0.52 & 0.48 & 0.48 \\
 & punctuation & 0.51 & 0.52 & 0.57 & 0.52 & 0.48 & 0.48 \\\cline{2-8}
 & \textbf{Average} & 0.51 & 0.52 & 0.61 & 0.53 & 0.48 & 0.46 \\ \midrule

\multirow{9}{*}{\shortstack{Mistral-7B-\\Instruct-v0.3}}
 & startend & 0.59 & 0.40 & 0.76 & 0.52 & 0.53 & 0.51 \\
 & detectable\_content & 0.53 & 0.43 & 0.72 & 0.49 & 0.53 & 0.53 \\
 & detectable\_format & 0.53 & 0.48 & 0.62 & 0.52 & 0.51 & 0.49 \\
 & language & 0.53 & 0.47 & 0.62 & 0.51 & 0.51 & 0.48 \\
 & change\_case & 0.50 & 0.46 & 0.58 & 0.51 & 0.51 & 0.46 \\
 & keywords & 0.52 & 0.48 & 0.58 & 0.51 & 0.51 & 0.47 \\
 & length\_constraints & 0.52 & 0.49 & 0.57 & 0.50 & 0.51 & 0.48 \\
 & punctuation & 0.52 & 0.49 & 0.58 & 0.51 & 0.50 & 0.48 \\\cline{2-8}
 & \textbf{Average} & 0.53 & 0.46 & 0.63 & 0.51 & 0.51 & 0.49 \\ \midrule

\multirow{9}{*}{\shortstack{Phi-3-mini-\\128k-instruct}}
 & startend & 0.47 & 0.39 & 0.70 & 0.65 & 0.48 & 0.48 \\
 & detectable\_content & 0.47 & 0.40 & 0.65 & 0.61 & 0.48 & 0.50 \\
 & detectable\_format & 0.48 & 0.43 & 0.64 & 0.55 & 0.52 & 0.52 \\
 & language & 0.49 & 0.42 & 0.65 & 0.56 & 0.51 & 0.52 \\
 & change\_case & 0.48 & 0.44 & 0.63 & 0.54 & 0.53 & 0.52 \\
 & keywords & 0.50 & 0.42 & 0.60 & 0.53 & 0.53 & 0.50 \\
 & length\_constraints & 0.50 & 0.44 & 0.58 & 0.53 & 0.52 & 0.51 \\
 & punctuation & 0.50 & 0.43 & 0.58 & 0.54 & 0.52 & 0.51 \\\cline{2-8}
 & \textbf{Average} & 0.49 & 0.42 & 0.63 & 0.56 & 0.51 & 0.51 \\ \bottomrule
\end{tabular}
}
\caption{Metrics for different models and instructions, showing verbal, perplexity, unnormalized perplexity, p(true)-normalized, p(true), and entropy.}
\label{tab:versionB}
\end{table}


